A New Optimization Layer for Real-Time Bidding Advertising Campaigns

While it is relatively easy to start an online advertising campaign, obtaining a high Key Performance Indicator (KPI) can be challenging. A large body of work on this subject has already been performed and platforms known as DSPs are available on the market that deal with such an optimization. From the advertiser's point of view, each DSP is a different black box, with its pros and cons, that needs to be configured. In order to take advantage of the pros of every DSP, advertisers are well-advised to use a combination of them when setting up their campaigns. In this paper, we propose an algorithm for advertisers to add an optimization layer on top of DSPs. The algorithm we introduce, called SKOTT, maximizes the chosen KPI by optimally configuring the DSPs and putting them in competition with each other. SKOTT is a highly specialized iterative algorithm loosely based on gradient descent that is made up of three independent sub-routines, each dealing with a different problem: partitioning the budget, setting the desired average bid, and preventing under-delivery. In particular, one of the novelties of our approach lies in our taking the perspective of the advertisers rather than the DSPs. Synthetic market data is used to evaluate the efficiency of SKOTT against other state-of-the-art approaches adapted from similar problems. The results illustrate the benefits of our proposals, which greatly outperforms the other methods.

==> acknowledge.tex <==
\section*{Acknowledgments}
\label{sec:acknowledgments}
We thank Soufian Aboulfaouz for numerous discussions (mainly concerning the market analysis as well as the \texttt{mab} and \texttt{lop} algorithms) and Yiming Wu for carefully reading and commenting the manuscript. 
We also want to express our appreciation to MediaMath for allowing us to use their platforms and for their technical assistance.


==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./pics/micchi.png}}]{Gianluca Micchi}
Born in 1987 in Italy, Gianluca got his piano diploma from the conservatory of Lucca, Italy, in 2008,
then his master's degree in physics at the University of Pisa, Italy, in 2012 with a theoretical work on the implementation of a qubit through a superconducting laser,
and finally a PhD in physics in 2016 at the University of Bordeaux, France, with a theoretical thesis about nano-electromechanical systems.
After that, he devoted himself to machine learning and artificial intelligence, working for Skylads since 2017.
% His interests lie in the advancement of artificial intelligence as a science, especially in connection to liberal arts.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./pics/soheily-khah.png}}]{Saeid Soheily-Khah}
graduated 
%from the Shahid Beheshti University of Tehran 
in computer engineering,
%in 2001. Then 
and received master degree in ”artificial intelligence $\&$
robotics” 
%from Azad University of Tehran - Iran 
in 2005. 
He then received his second master in information analysis and management from Skarbek university in Warsaw.%, Poland. %in 2013.
In %May 
2013, he joined to the LIG
%Laboratoire d'Informatique de Grenoble 
at Universit\'e Grenoble Alpes as a doctoral researcher. He successfully %defended his dissertation and 
got his Ph.D in Oct 2016.
In Nov 2016, he joined to the IRISA/Expression at Université Bretagne Sud as a postdoctoral researcher. Lastly, in Oct 2017, he joined Skylads %(artificial intelligence and big data analytics company) 
as a research scientist.
%His research interests are machine learning, data analysis and mining, cyber security system, anomaly detection, digital advertising and artificial intelligence.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./pics/jacob.png}}]{Jacob Turner} got his Ph.D. in mathematics at the Pennsylvania State University in 2015.
He then moved to Amsterdam to study combinatorial optimization algorithms under Alexander Schrijver before moving into industry as an algorithm developer with Skylads in 2017.
\end{IEEEbiography}

